Mining the Minoria: Unknown, Under-represented, and Under-performing Minority Groups

Due to a variety of reasons, such as privacy, data in the wild often misses the grouping information required for identifying minorities. On the other hand, it is known that machine learning models are only as good as the data they are trained on and, hence, may underperform for the under-represented minority groups. The missing grouping information presents a dilemma for responsible data scientists who find themselves in an unknown-unknown situation, where not only do they not have access to the grouping attributes but do not also know what groups to consider. This paper is an attempt to address this dilemma. Specifically, we propose a minority mining problem, where we find vectors in the attribute space that reveal potential groups that are under-represented and under-performing. Technically speaking, we propose a geometric transformation of data into a dual space and use notions such as the arrangement of hyperplanes to design an efficient algorithm for the problem in lower dimensions. Generalizing our solution to the higher dimensions is cursed by dimensionality. Therefore, we propose a solution based on smart exploration of the search space for such cases. We conduct comprehensive experiments using real-world and synthetic datasets alongside the theoretical analysis. Our experiment results demonstrate the effectiveness of our proposed solutions in mining the unknown, under-represented, and under-performing minorities.

==> proofs.tex <==
\section{Proof of Theorem~\ref{median_region_theorem}}
{\label{appendix:proofs}


\begin{theo}{\ref{median_region_theorem}}
    For a given median region with median $t_{m_f}$, the max skew direction $f^*$ either falls in the boundaries of this median region or it is equal to $\frac{(Q Q^\top)^{-1} q_{m_f}}{|(Q Q^\top)^{-1} q_{m_f}|}$.
\end{theo}

\begin{proof}
First, let us calculate the absolute value of $skew$ for an arbitrary given $f$:
\begin{align}
    skew(f) &= \Big\lvert \frac{mean(\mathcal{D}_f) - median(\mathcal{D}_f)}{sd(\mathcal{D}_f)} \Big\rvert
    \\  &= \Big\lvert \frac{mean(\mathcal{D})^T f - t_{m_f}^T f}{sd(\mathcal{D}_f)} \Big\rvert
    \\ &= \Big\lvert \frac{(mean(\mathcal{D}) - t_{m_f})^T f}{sd(\mathcal{D}_f)} \Big\rvert
\end{align}
The $sd(\mathcal{D}_f)$ is as follows:

\begin{align}
sd(\mathcal{D}_f) &= \sqrt{\frac{\sum^{n}_{i = 1} (mean(\mathcal{D}_f) - t_i^T f)^2}{n}} \\&= \sqrt{\frac{\sum^{n}_{i = 1} ((mean(\mathcal{D}) - t_i)^T f)^2}{n}}
\end{align}

Now, replacing $mean(\mathcal{D}) - t_i$ with $q_i$s, we have:

\begin{align}
    skew(f) &= \Big\lvert \frac{q_{m_f}^T f}{\sqrt{\frac{\sum^{n}_{i=1} (q_i^T f)^2}{n}}} \Big\rvert
\end{align}

Our objective is to find the $f^* = \argmax$ of $skew$:

\begin{align}
    f^* &= \argmax_f skew(f) \\
    &= \argmax_f skew(f)^2,
    \\ &=\argmax_f \frac{(q_{m_f}^T f)^2}{\sum^{n}_{i=1} (q_i^T f)^2}
    \\ &=\argmax_f \frac{(q_{m_f}^T f)^2}{f^T Q Q^T f}
\end{align}
Where $Q$, as defined above, is the matrix with $q_i$s as the columns. The vector $Q^T f$ will have $q_i^T f$ as it's elements. Dot product of this vector and it's transpose will give $\sum_{i=1}^{n} (q_i^T f)^2$. Let's define $g(f) = \frac{(q_{m_f}^T f)^2}{f^T Q Q^T f}$.



Now we calculate the derivative of the $\argmax$ with respect to $f$:
\begin{align}
    \frac{\partial g(f)}{\partial f} &= \frac{\partial (q_{m_f}^T f)^2}{\partial f} f^T Q Q^T f - \frac{\partial (f^T Q Q^T f)}{\partial f} (q_{m_f}^T f)^2
    \\
    &= 2 q_{m_f}^T f q_{m_f} (f^T Q Q^T f) 
    - 2 Q Q^T f (q_{m_f}^T f)^2
\end{align}

Solve the equation $\frac{\partial g(f^*)}{\partial f} = 0$:

\begin{align}
    \frac{\partial g(f^\star)}{\partial f} = 0 &\Leftrightarrow
    2 (q_{m_f}^T f^\star) (f^{\star T} Q Q^T f^\star) q_{m_f} = 2 (q_{m_f}^T f^\star)^2 Q Q^T f^\star \\
    &\Leftrightarrow
    (f^{\star T} Q Q^T f^\star) q_{m_f} = (q_{m_f}^T f^\star) Q Q^T f^\star \\
    & \Leftrightarrow f^\star = c (Q Q^T)^{-1} q_{m_f}
\end{align}

We assumed $q_{m_f}^T f^\star \neq 0$ to calculate the $\argmax$ of $skew$. In the last line, $c$ is a scalar value. So the direction of $f^*$ would be equal to $(Q Q^T)^{-1} q_{m_f}$. The unit vector for this direction would be $\frac{(Q Q^T)^{-1} q_{m_f}}{|(Q Q^T)^{-1} q_{m_f}|}$
\end{proof}

==> pseudocodes.tex <==
\section{Pseudo-codes}\label{appendix:pseudocodes}

% \begin{algorithm}[H]
% \caption{\warmup Algorithm for 2D}\label{alg:2d:naive}
% \begin{algorithmic}[1]
% \Procedure{2D\warmup}{$\dee, \theta$}
% \State $\mathcal{H} \gets Dual(\dee)$
% \State $\mathcal{A}_{\frac{n}{2}} \gets \mathcal{E}(\mathcal{H},\frac{n}{2})$\Comment{Ordered list of vertices in $\frac{n}{2}$th level of arrangement.}
% \State $Heap \gets [~]$\Comment{Initialize a max heap.}
% \For{$v$ in $\mathcal{A}_{\frac{n}{2}}$}
% \State $f \gets v / ||v||$\Comment{Get the direction of point $v$.}
% \State $skew \gets GetSkewNaive(\dee, f)$
% \State $Heap.push(<f, skew>)$\Comment{Push $f$ to a max heap based on the skew value.}
% \EndFor
% \State
% \State $Output \gets [~]$
% \While{$Output$ size is less that $l$}
% \State $f \gets Heap.pop()$\Comment{Get a candidate direction.}
% \State $T \gets \textit{p-}tail(f)$\Comment{$T$ is a candidate {\it \yoom} subset of $\dee$.}
% \If{$L_{T}(\theta) - L_{\dee}(\theta) > \tau$}
% \State $Output.append(f)$
% \EndIf
% \EndWhile
% \State \textbf{return} $Output$\Comment{Return the list of $l$ directions as candidate {\it \yoom}s.}

% \EndProcedure
% \State
% \Procedure{GetSkewNaive}{$\dee, f$}
% \State \textbf{return} $3(\mu(\dee_f) - \nu(\dee_f)) / \sigma(\dee_f)$\label{skew_naive_line}
% \EndProcedure
% \end{algorithmic}
% \end{algorithm}


% \begin{algorithm}[H]
% \caption{Generalized Ray Sweeping}\label{alg:2d:gen_ray_sweep}
% \begin{algorithmic}[1]
% \Procedure{GeneralizedRaySweeping}{$\dee, \theta$}
% \State $\mathcal{H} \gets Dual(\dee)$
% \State $\mathcal{G}_{\frac{n}{2}} = \mathcal{E}(\mathcal{H})$\Comment{The graph of k-level skeleton (vertices and edges).}\label{graph_line}
% \State $Heap \gets [~]$\Comment{Initialize a max heap.}

% \For{$v \in V(\mathcal{G}_{\frac{n}{2}})$ in a DFS traversal order}
% \State $f \gets v / ||v||$
% \State $skew = GetSkew(\dee, f)$\Comment{Use the aggregated values to get skew in constant time.}
% \State $Heap.push(<f, skew>)$
% \EndFor

% \State
% \State $Output \gets [~]$
% \While{$Output$ size is less that $l$}
% \State $f \gets Heap.pop()$
% \State $T \gets \textit{p-}tail(f)$
% \If{$L_{T}(\theta) - L_{\dee}(\theta) > \tau$}
% \State $Output.append(f)$
% \EndIf
% \EndWhile
% \State \textbf{return} $Output$\Comment{Return the list of $l$ directions as candidate {\it \yoom}s.}

% \EndProcedure
% \end{algorithmic}
% \end{algorithm}


\begin{algorithm}[H]
\caption{Smart Exploration}\label{alg:md:smart_exploration}
\begin{algorithmic}[1]
\Procedure{SmartExplore}{$\dee, h_{\theta}, \mathcal{K}, \mathcal{K}^{\prime}$}\Comment{$h_{\theta}$ is the trained model on $\dee$.}
\State $\dee_{sorted} \gets sort(\dee, L_{\theta})$\Comment{Sorts $\dee$ based on the loss function $L_{\theta}$ (descending).}
\State $S \gets \textit{First } \mathcal{K} \textit{ portion of } D_{sorted}$\Comment{$S$ is the error region.}
\State $D^S \gets sample(S)$\Comment{Down sample the error region uniformly.}
\State $D^{!S} \gets sample(\dee \setminus S)$
\State
\State $Heap \gets [~]$\Comment{Initialize a max heap.}
\For{all vectors $v \in \{s - t | s \in D^S, t \in D^{!S}\}$}
\State $f \gets v / ||v||$
\State $skew = GetSkew(\dee, f)$
\State $Heap.push(<f, skew>)$
\EndFor

\State
\State $Output \gets [~]$
\While{$Output$ size is less that $l$}
\State $f \gets Heap.pop()$
\State $T \gets \textit{p-}tail(f)$
\State $T_{err} \gets \textit{First $\mathcal{K}^{\prime}$ portion of $sort(T, L_{\theta})$}$\label{error_points_of_tail}\Comment{Keep the challenging points of the tail}
\If{$L_{T_{err}}(\theta) - L_{\dee}(\theta) > \tau$}
\State $Output.append(f)$
\EndIf
\EndWhile
\State \textbf{return} $Output$\Comment{Return the list of $l$ directions as candidate {\it \yoom}s.}

\EndProcedure
\end{algorithmic}
\end{algorithm}
